LlaMaVAE: Guiding Large Language Model Generation via Continuous Latent Sentence Spaces

Deep generative neural networks, such as Variational AutoEncoders (VAEs), offer an opportunity to better understand and control language models from the perspective of sentence-level latent spaces. To combine the controllability of VAE latent spaces with the state-of-the-art performance of recent large language models (LLMs), we present in this work LlaMaVAE, which combines expressive encoder and decoder models (sentenceT5 and LlaMA) with a VAE architecture, aiming to provide better text generation control to LLMs. In addition, to conditionally guide the VAE generation, we investigate a new approach based on flow-based invertible neural networks (INNs) named Invertible CVAE. Experimental results reveal that LlaMaVAE can outperform the previous state-of-the-art VAE language model, Optimus, across various tasks, including language modelling, semantic textual similarity and definition modelling. Qualitative analysis on interpolation and traversal experiments also indicates an increased degree of semantic clustering and geometric consistency, which enables better generation control.

==> sections/disentang_framework.tex <==
%\input{tikz/models.tex}

\section{Background} \label{sec:disentang}

\paragraph{Latent semantic space}

\citep{zhang2022} demonstrates that semantic role of explanations can be separated in a latent space modeled using Optimus \cite{li2020optimus}. Each \textit{role -- content word} combination is described by a hypersolid (region) in the latent space. For example, some semantic clusters, such as \textit{ARG1-shelter} and \textit{ARG1-warmth} (``shelter'' or ``warmth'' as direct object) around the cluster \textit{ARG0-animal} (``animal'' as subject). Because of this geometric property, they can control the generation of explanations by manipulating the latent vectors over different clusters. Next, they adopt flow-based INN to learn more separate role-content clusters, which indicates the disentanglement of semantic information. However, those approaches inevitably lead to loss of semantic information because of the sentence bottleneck of VAE setting. In our work, we investigate VQVAE in learning disentangled representation space, which can avoid this issue and provide better semantic control to decoder.

\paragraph{VQVAE} \citet{van2017neural} put forward the VQVAE for learning discrete latent space of image. It can avoid the issue ``posterior collapse'', which the latent representations from encoder are ignored in decoder, suffered in the training process of VAE \cite{kingma2013auto}. In detail, they define a latent embedding space $z \in R^{K \times D}$ where $K$ and $D$ represent the size of that space and its dimension, respectively. Given an input $x$, the Encoder $E$ first encode $x$ into its vector representation $E(x)$. Then, the model selects the nearest latent representation $z_k$ from predefined latent space via $L2$ distance that is $k = \operatorname{argmin}_j|| e^{w_i} - z^j ||_2, j \in [1, ..., D] $ as the input of Decoder $D(z_k)$. To avoid the no-differentiable $E$ derived from argmin, straight-through gradient estimation is considered to map the gradient from $E(x)$ to $D(z_k)$ directly by bypassing the $z_k$ and update $z_k$ by minimizing the $L2$ distance between $E(x)$ and $z_k$, which can be described as: $(\text{sg}[E(x)] - z_k)^2$ where $\text{sg}$ is stop gradient operation. Finally, to assure the $E$ can choose the latent embedding from constrained $R^{K \times D}$ rather than learn latent embedding directly as without latent space the model connected by $E$ and $D$ can lead to better performance, a commitment loss is described to constraint the $E$ close to $z$. The final objective function can be described as:
\[
\begin{aligned}
\mathcal{L}_{VQVAE} = P(x|D(z_k)) + \left ( \text{sg}[E(x)] - z_k \right )^2 \\ \nonumber
+ \beta \left ( E(x) - \text{sg}[z_k] \right )^2
\end{aligned}
\]



==> sections/eval.tex <==
% \section{Controllability Evaluation} \label{sec:eval}






==> sections/explanation_control.tex <==
\subsection{Controllable Explanation Generation}

\noindent Considering the verified hypotheses in the previous section and their geometrical interpretation, we investigate a way to control the generation of explanations by manipulating the movement of vectors in the latent space without direct intervention, i.e., specifying a traversal learning method. Specifically, we first implement a decision tree as a binary classifier to classify the sentences from two different regions (clusters role-content). Then, we visualize that tree where each non-leaf node contains the specific value range of its corresponding dimension and each leaf node contains the number of sentences that fall under this node. Therefore, we can follow a path of that tree to move across the clusters of the input sentences. In figure \ref{fig:decision_tree}, for example, we can move the sentence in cluster 0 to 4 by modifying the values started from \textit{dim 27 <= -0.493}, ..., ending at \textit{dim 21 <= -0.891}. As a consequence, the node thresholds also define a boundary between latent space regions.
\vspace{0.3cm}

\begin{figure}[ht!]
\begin{center}
    \includegraphics[scale=0.35]{figs/decision_tree.png}
    \caption{Example of a path in decision tree where C0 and C4 are two topic-role clusters.}
    \label{fig:decision_tree}
 \end{center}
\end{figure}

\noindent \textbf{Traversal between topics} ~~As illustrated in table \ref{tab:movement_topic_example} we can observe that the cluster of the generated sentence changes as the values of different dimensions change sequentially (e.g., the first three sentences hold the same characteristic \textit{if ... then ...} as the input. The remaing sentences gradually move closer to the target characteristics, such as \textit{is}, in cluster 4). The accuracy (\textit{classifier separability}), precision, recall (\textit{classifier density}), and f1 score  of that decision tree are 0.58, 0.57, 0.55, 0.54, respectively, which indicate a low level of separability w.r.t. topics. Moreover, we can find that the sentences can hold the subject, \textit{something}, during the movement, which corroborates our aforementioned hypothesis ($\#2$), in which both role and content information are components of the latent space encoding. 
\vspace{0.3cm}
\input{tables/movement_between_topics.tex}
\vspace{0.3cm}
\noindent \textbf{Traversal between predicates} ~~Table \ref{tab:movement_verb_example} shows an example of movement between verbs (\textit{cause} and \textit{mean}). From it, we can observe that the predicate is modified from \textit{causes} to \textit{mean}. In the traversal process, some sentences fall into the \textit{is} region, as the \textit{is} and the \textit{mean} regions have a large overlap in latent space. 
Additionally, classifier separability and density are 0.87 and 0.92
%the accuracy, precision, recall, and f1 score of that decision tree are 0.87, 0.83, 0.92, 0.88, 
respectively, indicating high separability w.r.t. predicate regions. Moreover, we calculate the ratio of the generated sentences that hold the expected predicate (\textit{cross-region consistency}), \textit{mean}, from 100 sentences with predicate \textit{cause}. The ratio is 0.71, which indicates that the decision tree is a reliable way to control the movement of sentences.4

\input{tables/movement_between_verbs.tex}
\vspace{0.3cm}
\noindent \textbf{Traversal between arguments}~~Table \ref{tab:movement_arg_example} shows the example of movement from argument \textit{water} to \textit{something}.  It produces a similar observation as the predicate case. The ARG1 can be modified from \textit{water} to \textit{something} following its path. Classifier separability and density are 0.95 and 0.48
%accuracy, precision, recall, and f1 score are 0.95, 0.5, 0.48, 0.49,
respectively, indicating high separability, albeit hindered by sparsity across the argument regions.

\input{tables/movement_between_arguments.tex}

% Instead of employing decision tree for moving the sentences over clusters in latent space, we can also utilize it to reveal the information in a cluster. Therefore, we next explore more information of cluster with arg1 \textit{water}. 
% \vspace{0.3cm}
% \noindent \textbf{Case study of water cluster}~~Figure \ref{fig:case_study_water} displays the path of arg1 \textit{water} in decision tree. There are three main paths to arg1 \textit{water}. Firstly, we investigate the difference of sentences in the left and right paths. As illustrate in table \ref{tab:case_study_water} 

% \begin{figure}[ht!]
% \begin{center}
%     \includegraphics[scale=0.35]{figs/case_study_water.png}
%     \caption{Decision tree of \textit{water} vs \textit{something}.}
%     \label{fig:case_study_water}
%  \end{center}
% \end{figure}
% \input{tables/case_study_water.tex}
% \vspace{0.3cm}





==> sections/inference.tex <==
\subsection{Natural Language Inference}
With the possibility of granular control over the latent space semantics, the next step would be to achieve the effect of reasoning through the movement of the sentence in the latent space. Therefore, we next focus on an extrinsic natural language inference task: generating a conclusion given by two premises. By modeling a transformation from any two given points (the premises) into one (the conclusion) in this space, we can find connections between the disentangled space properties and explanatory inference.

We encode two premises into the latent space, separately. Then, we employ a multi-layer perceptron to learn the transformation function from premises to the conclusion. During training, we only fine-tune the $\mu$, $\sigma$, and inference layers and freeze the remaining layers in Optimus. The initial weights are from unsupervised, supervised, and conditional frameworks. TODO

\vspace{0.3cm}
\noindent
\textbf{Quantitative evaluation}~~Table~\ref{tab:results_generation} compares the perplexity of conclusion generation between T5, BART, and the disentangled Optimus with inference module. From it, we can observe that the non-VAE models (T5 and Bart) outperform VAE model (Optimus) with a big gap, indicating that the information relevant to encoding both premises and conclusions for reconstruction (the VAE compression) is at least partly disjoint from the information relevant to map the premises to conclusions. Table~\ref{tab:generation_examples} shows some examples generated from baselines.

\input{tables/generation_results.tex}
% \vspace{-1cm}
% \noindent
% \textbf{Quantitative evaluation}~~Table \ref{tab:generation_examples} shows some examples generated from baselines. We found that Optimus with the inference network cannot learn a proper transformation from premises to conclusion automatically. Therefore, we will explore how can manually operate the movement of vector to achieve inference in the future. 

\input{tables/generation_examples.tex}

% \begin{figure}[ht!]
% \begin{center}
%     \includegraphics[scale=0.34]{figs/inference.png}
%     \caption{Process of inference in the latent space of Optimus.}
%     \label{fig:inference}
%  \end{center}
% \end{figure}
% Table~\ref{tab:generation_examples} shows some conclusion generated from baselines. From them, we can find that LM (T5 and BART) always perform better than VAE model. Among them, T5 outperforms others with a big gap.







==> sections/inference_impl.tex <==
\subsection{Implications to inference}
The degree of semantic and structural separability and consistency evaluated, and the quality of explanation control demonstrated at the semantic role level suggests the existence of a family of functions $\mathcal{I}: Z^n \rightarrow Z$, where $Z$ is the encoder latent space, mapping any given set of premises to a conclusion via a composition of structural and semantic transformations, leading to the language processing architecture illustrated in Figure~\ref{fig:model_infer}. A model for finding the optimal function should be the object of future research.

\begin{figure}[ht!]
    \centering
    \includegraphics[scale=0.55]{figs/model_infer.pdf}
    \caption{Inference model architecture.}
    \label{fig:model_infer}
\end{figure}

==> sections/limitations.tex <==
\section*{Limitations}
Despite the increased degree of separability and generation control achieved for the explanatory sentences by flow-based INN, it is only the first step into connecting disentangled semantic roles. How to achieve natural language inference through this latent space with geometric properties still needs to be explored.

==> sections/metrics.tex <==
\section{Disentanglement Metrics} \label{sec:metrics}

\begin{enumerate}
    % \item $z_{diff}~accuracy$~\cite{higgins2016beta}: The accuracy of a predictor for $p(y|z^b_{diff})$, where $z^b_{diff}$ is the absolute linear difference between the inferred latent representations for a batch $B$ of latent vectors, written as a percentage value. Higher values imply better disentanglement.

    \item $z_{min\_var}~error$~\cite{kim2018disentangling}: For a chosen factor k, data is generated with this factor fixed but all other factors varying randomly; their representations are obtained, with each dimension normalised by its empirical standard deviation over the full data (or a large enough random subset); the empirical variance is taken for each dimension of these normalised representations. Then the index of the dimension with the lowest variance and the target index k provide one training input/output example for the classifier. Thus, if the representation is perfectly disentangled, the empirical variance in the dimension corresponding to the fixed factor will be 0. The representations are normalised so that the arg min
    is invariant to rescaling of the representations in each dimension. Since both inputs and outputs lie in a discrete space, the optimal classifier is the majority-vote classifier, and the metric is the error rate of the classifier. Lower values imply better disentanglement.

    \item Mutual Information Gap ($MIG$)~\cite{chen2018isolating}: The difference between the top two latent variables with the highest mutual information. Empirical mutual information between a latent representation $z_j$ and a ground truth factor $v_k$, is estimated using the joint distribution defined by  $q(z_j, v_k) = \sum_{n=1}^{N}{p(v_k)p(n|v_k)q(z_j|n)}$. A higher mutual information implies that $z_j$ contains a lot of information about $v_k$, and the mutual information is maximal if there exists a deterministic, invertible relationship between $z_j$ and $v_k$. MIG values are in the interval [0, 1], with higher values implying better disentanglement.

    \item \textit{Modularity}~\cite{ridgeway2018learning}: The deviation from an ideally modular case of latent representation. If latent vector dimension $i$ is ideally modular, it will have high mutual information with a single factor and zero mutual information with all other factors. A deviation $\delta_i$ of 0 indicates perfect modularity and 1 indicates that this dimension has equal mutual information with every factor. Thus, $1 - \delta_i$ is used as a modularity score for vector dimension i and the mean of $1 - \delta_i$ over $i$ as the modularity score for the overall representation. Higher values imply better disentanglement.

    % \item \textit{Explicitness}~\cite{ridgeway2018learning}: Mean of the ROC area-under-the-curve ($AUC_{jk}$) of a one-versus-rest logistic-regression classifier that takes the latent vectors as input and has factor values as targets, over a factor index $j$ and an index $k$ on values of factor $j$. Represents the coverage of the representation, in other words, how well each factor is represented. Higher values imply better disentanglement.

    \item \textit{Disentanglement Score}~\cite{eastwood2018framework}: The degree to which a representation factorises or disentangles the underlying factors of variation, with each variable (or dimension) capturing at most one generative factor. It is computed as a weighted average of a disentanglement score $D_i = (1 -  H_K(P_i.))$ for each latent dimension variable $c_i$, on the relevance of each $c_i$, where $H_K(P_i.)$ denotes the entropy and $P_{ij}$ denotes the 'probability' of $c_i$ being important for predicting $z_j$. If $c_i$ is important for predicting a single generative factor, the score will be 1. If $c_i$ is equally important for predicting all generative factors, the score will be 0. Higher values imply better disentanglement.

    \item \textit{Completeness Score}~\cite{eastwood2018framework}: The degree to which each underlying factor is captured by a single latent dimension variable. For a given $z_j$ it is given by $C_j = (1 - H_D(\tilde{P}.j))$, where $H_D(\tilde{P}.j) = -\sum_{d=0}^{D - 1}{\tilde{P}_{dj} log_D \tilde{P}_{ij}}$ denotes the entropy of the $\tilde{P}.j$ distribution. If a single latent dimension variable contributes to $z_j$'s prediction, the score will be 1 (complete). If all code variables contribute equally to $z_j$'s prediction, the score will be 0 (maximally over-complete). Higher values imply better disentanglement.

    \item \textit{Informativeness Score}~\cite{eastwood2018framework}: The amount of information that a representation captures about the underlying factors of variation. Given a latent representation $c$, It is quantified for each generative factor $z_j$ by the prediction error $E(z_j , \hat{z}_j)$ (averaged over the dataset), where $E$ is an appropriate error function and $\hat{z}_j = f_j(c)$. Lower values imply better disentanglement.
\end{enumerate}

==> sections/qualitative.tex <==
\subsection{Qualitative Evaluation}
We analyse the representations of the trained models in terms of their disentanglement and composition, by applying three different techniques 1) traversals of the latent space, 2) latent space arithmetic, 3) encoding interpolation. %4) encoding visualization with dimensionality reduction.

\noindent
\textbf{Latent space traversals}
Traversal evaluation is a standard procedure with image disentanglement~\citep{higgins2016beta,kim2018disentangling}. The traversal of a latent factor is obtained as the decoding of the vectors corresponding to the latent variables, where the evaluated factor is changed within a fixed interval, while all others are kept fixed. If the representation is disentangled, when a latent factor is traversed, the decoded sentences should only change with respect to that factor. This means that after training the model we are able to probe the representation for each latent variable. In the experiment, the traversal is set up from a starting point given by a ``seed'' sentence. As illustrated in Table~\ref{tab:trav_examples} ...

\input{tables/trav_examples.tex}

% \noindent
% \textbf{Latent space arithmetic}
% In this experiment, the latent vectors for two sentences are added, subtracted or averaged, and then the resulting vectors are traversed. The sentence pairs are different by a single term, so that we can observe the latent variables affected by the change, and how they are affected. As illustrated in Table~\ref{tab:arith_examples}, ...

% \input{tables/arith_examples.tex}

\noindent
\textbf{Interpolation}
In this experiment, we demonstrate the ability of autoencoder models to provide smooth transition between latent space representations of sentences~\citep{bowman2016generating}. In practice, the interpolation mechanism takes two sentences $ x_1 $ and $ x_2 $, and uses their posterior mean as the latent features $ z_1 $ and $ z_2 $, respectively. It interpolates a path $ z_t = z_1 \cdot (1 - t) + z_2 \cdot t  $  with $ t $ increased from $ 0 $ to $ 1 $ by a step size of $ 0.1 $.  As a result, $ 9  $ sentences are generated on each interpolation step. In Table~\ref{tab:interpol_examples} we provide qualitative results with latent space interpolation on ...

\input{tables/interpol_examples.tex}

Based on those three experiments, the composition of such latent space could be conceptualised as in the projection illustrated in Figure~\ref{fig:latent_concept}.

\begin{figure}[ht]
    \centering
    % \includegraphics[scale=0.5]{figs/latent_diagram}
    \caption{Conceptualisation of a two-dimension cut of the latent space, applied to the first example in Table~\ref{tab:interpol_examples}.}
    \label{fig:latent_concept}
\end{figure}

\begin{figure}[t]
    % \includegraphics[scale=0.23]{figs/umap_all}
    \caption{UMAP plot of latent representations from Unsupervised VAE (U), DSR supervision (S) and Conditional VAE (C) (Top: LSTM, Bottom: Optimus).}
    \label{fig:umap}
\end{figure}

\paragraph{UMAP plot}
\textit{UMAP} (Uniform Manifold Approximation and Projection)~\cite{mcinnes2018umap} is a popular method for non-linear dimensionality reduction, that allows the visualization of complex high-dimensional feature spaces, such as the representation space produced by a VAE. Figure~\ref{fig:umap} presents a 2D plot of UMAP transformations for both baselines under three training frameworks, .... t-SNE transformations are also performed and the plots are presented in the supplemental material (Appendix~\ref{sec:apd_exp_res}).



==> sections/quantitative.tex <==
\subsection{Quantitative Evaluation}
In this experiment we probe the representation learned by the proposed VAE models using eight popular quantitative metrics for disentanglement, namely: z-diff~\citep{higgins2016beta}, z-min-var~\citep{kim2018disentangling}, Mutual Information Gap (MIG)~\citep{chen2018isolating}, Modularity \& Explicitness~\citep{ridgeway2018learning}, and from~\citep{eastwood2018framework}(disentanglement, completeness, informativeness). Further details about the metrics are provided in Appendix~\ref{sec:metrics}.

\noindent
\textbf{Experimental Setup}
We evaluate VAE (U), DSR VAE (S) and CVAE (C) on ... Evaluation is performed under the framework explained in Section~\ref{sec:eval}. Each combination of VAE architecture, generative factor grouping and representation size was trained and quantitatively tested, by calculating the previously mentioned disentanglement metrics. For computing the metrics we follow the experiments of~\citet{zhang2021unsupervised}.

\noindent
\textbf{Analysis}
The results presented in Tables~\ref{tab:trav_examples},~\ref{tab:interpol_examples}, and ~\ref{tab:all_metrics} show that, specially when using the Optimus model:

\input{tables/all_ds_by_exp.tex}

Results discussion
...


%In conclusion, this analysis places DSR-based generative factors as a promising, yet complex, target for disentanglement on Natural Language definitions, as they encode both meaning and structure in each category.






%\begin{figure}[h]
% \includegraphics[scale=0.5]{figs/wn_zdiff_dims}
% \caption{Z Diff mean on Wordnet dataset.}
% \label{fig:factors_analysis}
%\end{figure}

==> tables/arithmetic.tex <==
% traversals results
\begin{table}[ht!]
\centering
\begin{tcolorbox}[fontupper=\small, fontlower=\small]

\textcolor{blue}{El niño causes drought in the western United States} \\
1. El niño causes varied water tematures in the western United States \\
2: El niño causes varied water temperature \\
3: El niño causes varied rainfall \\
4: drought may cause the erosion in agricultural grounds \\
5: subduction may cause volcano eruption \\
6: subduction is when one tectonic plate moves under another tectonic plate \\
7: water above freezing is located in the solution \\
8: water in the liquid state is less dense than water in solid state \\
9: water is in the liquid state called water \\
10: water is in the liquid state \\
% 1: El niño causes flooding in the western Pacific \\
% 2: \textcolor{red}{El niño causes flooding in the western United States} \\
% 3: El niño causes flooding on the Pacific coast of South America \\
% 4: El niño causes surface flooding \\
% 5: water is in the liquid state, called liquid water, for temperatures between 0 c and 100 c \\
% 6: \textcolor{red}{water is in the liquid state, called liquid water, for temperatures between 273 and 538 c} \\
% 7: \textcolor{red}{water is in the liquid state called ice} \\
% 8: water is in the liquid state called liquid water \\
% 9: water is at the bottom of an ocean \\
% 10: water is in the liquid state called water \\
\textcolor{blue}{water is in the liquid state called water}
% 1: forming sedimentary rock requires burying sediments \\
% 2: forming sedimentary rock requires burying the rock \\
% 3: forming sedimentary rock means sediment is compacted \\
% 4: forming a fossil requires the process of burial \\
% 5: an example of collecting data in an arctic animal ecosystem requires measuring animal habitats \\
% 6: an example of managing the use of a resource is replacing that resource \\

% 1: forming sedimentary rock requires compacting and cementing the layers \\
% 2: creating rocks requires deposition and burial \\
% 3: forming sedimentary rock requires burying  \\
% 4: forming sedimentary rock requires compacting the materials \\
% 5: producing something means ( producing ; delivering ) something \\
% 6: something combining two substances chemically is similar to producing two substances chemically \\
% 7: an example of managing the use of trees is replacing trees \\
% 8: an example of managing the use of a resource is replacing that resource \\
% 9: an example of managing the use of trees is replacing trees \\
% 10: an example of managing the use of something is using less of that something \\

% \textcolor{blue}{an example of managing the use of a resource is replacing that resource}
\end{tcolorbox}
\caption{LlaMaVAE: latent arithmetic.}
\label{tab:arithmetic}
\end{table}

==> tables/disentangled_metrics.tex <==
\begin{table}[ht!]
\scriptsize
\setlength\tabcolsep{2.5pt}
\small
\centering
\resizebox{7.8cm}{!}{
\renewcommand\arraystretch{1.3}
\begin{tabular}{llll}
\toprule
Metrics & Optimus(32, U) & Optimus(32, S) & Optimus(32, C) \\ \hline
z-min-var $\downarrow$ &  .451 & .453 & .401 \\ 
MIG  & .027 & .067 & .039 \\ \hline
Metrics & INN(U) & T5VQVAE(small) & T5VQVAE(base) \\ \hline
z-min-var $\downarrow$ &  .350 & \\ 
MIG  & .491 & \\ 
\toprule
\end{tabular}
}
\caption{Disentanglement evaluation.} \label{tab:disentangled_metrics}
\end{table}

==> tables/fur_con.tex <==
\begin{table}[ht!]
\begin{tcolorbox}[fontupper=\small, fontlower=\small, title=Further specification and Conjunction]
P1: a plant requires energy \textcolor{blue}{to make food} \\
P2: plants get energy from sunlight \\
Pred: plants get energy from sunlight \textcolor{blue}{to make food} \\

P1: a mountain is \textcolor{blue}{made of rocks} \\
P2: a mountain range contains mountains \\
Pred: a mountain range contains mountains \textcolor{blue}{made of rocks} \\

P1: a dinosaur is a kind of \textcolor{blue}{animal} \\
P2: dinosaurs are cold-blooded \\
Pred: dinosaurs are cold - blooded \textcolor{blue}{animals} \\

P1: \textcolor{blue}{gravity causes} orbits \\
P2: planets in the solar system orbit the sun \\
Pred: gravity causes planets in the solar system to orbit the sun \\

P1: scattering light \textcolor{blue}{decreases visibility} \\
P2: water droplets scatter light \\
Pred: water droplets scattering light \textcolor{red}{decreases air droplets} \\
Gold: water droplets scattering light decreases the visibility
\tcblower
P1: sound travels \textcolor{blue}{slowest through gas} \\
P2: sound travels \textcolor{blue}{fastest through solid} \\
Pred: sound waves travel fastest \textcolor{red}{through gas and gas} \\
Gold: sound travels fastest through solid and slowest through gas \\

P1: matter in the solid phase has definite \textcolor{blue}{volume} \\
P2: matter in the solid phase has definite \textcolor{blue}{shape} \\
Pred: matter in the solid phase has definite shape and volume \\

P1: a plant requires \textcolor{blue}{nutrients} from soil to grow \\
P2: a plant requires \textcolor{blue}{water} from soil to grow \\
Pred: a plant requires water and nutrients from soil to grow \\

P1: a hurricane has \textcolor{blue}{high wind speed} \\
P2: a hurricane has \textcolor{blue}{large amount of rain} \\
Pred: a hurricane has high wind speed and large amount of rain \\


P1: fungi \textcolor{blue}{can be multicellular} \\
P2: fungi \textcolor{blue}{have no chlorophyll} \\
Pred: fungi have no chlorophyll and can be multicellular \\
\end{tcolorbox}
\caption{T5VQVAE(base): quasi-symbolic inference examination in AutoEncoder (Top: further specification, Bottom: conjunction).}
\label{tab:quasi}
\end{table}

==> tables/interpolation_more.tex <==
% traversals results
\begin{table}[ht!]
\centering
\begin{tcolorbox}[fontupper=\small, fontlower=\small] %, middle=0.3cm 
\underline{\textbf{Source: some birds have a speckled brown color}} \\ \\
1. \textcolor{blue}{some birds} \ul{have} \textcolor{orange}{a speckled brown color} \\
2. \textcolor{blue}{some birds} \ul{live in} \textcolor{orange}{an arctic environment} \\
3. \textcolor{blue}{some arctic animals} \ul{live in} \textcolor{orange}{a speckled green environment} \\
4. \textcolor{blue}{arctic animals} \ul{live in} \textcolor{orange}{an arctic environment} \\ \\

1. \textcolor{blue}{some birds} \ul{have} \textcolor{orange}{a speckled brown color} \\
2. \textcolor{blue}{some birds} \ul{have} \textcolor{orange}{scales} \\
3. \textcolor{blue}{some birds} \ul{are} \textcolor{orange}{scaled} \\
4. \textcolor{blue}{some birds} \ul{are} \textcolor{orange}{herbivores} \\
5. \textcolor{blue}{some eagles} \ul{live in} \textcolor{orange}{open environments} \\
6. \textcolor{blue}{some birds} \ul{are} \textcolor{orange}{eagles} \\
7. \textcolor{blue}{some birds} \ul{are} \textcolor{orange}{herbivores} \\
8. \textcolor{blue}{eagles} \ul{live in} \textcolor{orange}{an arctic environment} \\
9. \textcolor{blue}{arctic animals} \ul{live in} \textcolor{orange}{an arctic environment} \\

\underline{\textbf{Target: arctic animals live in an arctic environment}}
\end{tcolorbox}
\caption{Interpolation for T5VQVAE (top) and Optimus (bottom) where \textcolor{blue}{blue}, \ul{underline}, and \textcolor{orange}{orange} represent subject, verb, and object, respectively.}
\label{tab:interpolation_more}
\end{table}

==> tables/more_quasi_symbolic.tex <==
% traversals results
\begin{table}[ht!]
\centering
% \begin{tcolorbox}[sidebyside]
\begin{tcolorbox}[fontupper=\small, fontlower=\small, title=Further specification and Conjunction] %, middle=0.3cm 
% \begin{multicols}{2}
P1: coal is a \textcolor{blue}{nonrenewable} resource \\
P2: coal is a kind of \textcolor{blue}{natural} resource \\
Pred: coal is a kind of \textcolor{blue}{nonrenewable natural} resource \\

P1: water \textcolor{blue}{contains dissolved oxygen} \\
P2: water is a part of an environment \\
Pred: water is a part of an environment that \textcolor{blue}{contains dissolved oxygen}
% P1: the earth \textcolor{blue}{rotates on its tilted axis} \\
% P2: earth is a kind of planet \\
% Pred: earth \textcolor{blue}{being on its tilted axis} is a kind of planet \\
% Gold: earth is a planet that \textcolor{blue}{rotates on its tilted axis}
% P1: light is a kind of \textcolor{blue}{energy} \\
% P2: sunlight is a kind of \textcolor{blue}{light} \\
% Pred: sunlight is a kind of \textcolor{red}{energy} \\
% Gold: sunlight is a kind of \textcolor{blue}{light energy}
\tcblower

P1: an arctic environment is \textcolor{blue}{white in the winter} \\
P2: an arctic environment is \textcolor{blue}{dark gray or brown in the summer} \\
Pred: an arctic environment is \textcolor{blue}{dark gray or brown in the summer} and \textcolor{blue}{white in the winter} \\

P1: \textcolor{blue}{sedimentary} is a class of rock \\
P2: \textcolor{blue}{metamorphic} is a class of rock \\
Pred: \textcolor{blue}{metamorphic} is a class of rock and \textcolor{blue}{sedimentary} rock \\
Gold: \textcolor{blue}{sedimentary and metamorphic} are different classes of rock

\end{tcolorbox}
\caption{T5VQVAE(base): Further specification or conjunction inference (Top: \textit{further specification}, bottom: \textit{conjunction}).}
\label{tab:fur_or_con}
\end{table}

==> tables/semantic_metrics_nli.tex <==
% \begin{center}
\begin{table}[ht!]
\scriptsize
\setlength\tabcolsep{2.5pt}
\resizebox{7.8cm}{!}{
% \small
% \centering
\renewcommand\arraystretch{1.3}
\begin{tabular}{llllll}
\toprule
Baseline & BLEU & Cosine & BLEURT & Loss $\downarrow$ & PPL $\downarrow$ \\ \hline
T5(small) & 0.54 & 0.96 & 0.22 & 0.69 & 1.99 \\
T5(base) & \textbf{0.57} & \textbf{0.96} & \textbf{0.33} & \textbf{0.61} & \textbf{1.84} \\
Bart(base) & 0.54 & 0.96 & 0.17 & 0.63 & 1.87 \\
FlanT5(small) & 0.22 & 0.89 & -1.33 & 0.99 & 2.69 \\ \hline 
Optimus(32) & 0.08 & 0.74 & -1.21 & 0.82 & 2.27 \\
T5VQVAE(small) & 0.11 & 0.73 & -1.23 & 0.85 & 2.33 \\
T5VQVAE(base) & 0.46 & 0.94 & 0.10 & 0.84 & 2.31 \\ \toprule
\end{tabular}
}
\caption{Quantitative evaluation of inference task.} \label{tab:metrics_inf}
\end{table}
% \end{center}
